DisFace3DNet: Explainable Facial Attractiveness Prediction via 3D Component Disentanglement

Facial attractiveness prediction usually assigns one overall rating, leaving the roles of shape, appearance, and viewing conditions implicit. We propose DisFace3DNet, which uses 3D component disentanglement to learn seven component reference scores from overall ratings with auxiliary weak semantic supervision, without human-labeled component targets. Designated 3D representations and image cues feed jointly learned routes for identity, skin, hair, light, background, expression, and pose. A constrained fit then combines five static and two signed dynamic scores into the overall rating, exposing each component's numerical contribution and supporting component-specific comparisons across images. On SCUT-FBP5500, DisFace3DNet achieves a Pearson correlation of $0.8904\pm0.0063$ (mean $\pm$ standard deviation across five folds) with average human ratings; its component terms reconstruct every held-out prediction to numerical precision. Skin, hair, and facial shape account for the largest component-wise prediction variation. Human evaluation supports the score directions for facial shape, skin, and hair; expression agreement is weaker. DisFace3DNet thus connects overall prediction to quantitative analysis of the facial and contextual cues entering each estimate.

==> main_counts.tex <==
\setcounter{figure}{10}
\setcounter{table}{3}
\setcounter{equation}{20}


==> main_refs.tex <==
% Generated by joint build; use starred cross-document references.
\newlabel{main:sec:introduction}{{I}{1}{Introduction}{section.1}{}}
\newlabel{main:fig:prediction_explanation}{{1}{2}{Prediction and explanation interfaces. (a) Overall prediction through regression, distribution learning, or ranking~\cite {eisenthal2006facial,fan2018label,lyu2024ranking}. (b) Post-hoc explanation~\cite {Selvaraju2017GradCAM,Chattopadhyay2018GradCAMPlusPlus,Wang2020ScoreCAM}, illustrated by Grad-CAM. (c) DisFace3DNet uses separate component predictors to produce component reference scores, which are combined by weighted fusion into the overall rating. Head renderings illustrate the components; scores are symbolic. $E$ and $D$ denote encoder and decoder}{figure.1}{}}
\newlabel{main:sec:related_work}{{II}{2}{Related Work}{section.2}{}}
\newlabel{main:sec:method}{{III}{3}{Method}{section.3}{}}
\newlabel{main:sec:component_disentanglement}{{\mbox  {III-B}}{3}{Component Disentanglement}{subsection.3.2}{}}
\newlabel{main:sec:group_conditioning}{{\mbox  {III-C}}{3}{Benchmark-Group Conditioning}{subsection.3.3}{}}
\newlabel{main:fig:architecture}{{2}{4}{Architecture of DisFace3DNet. Component Disentanglement provides designated inputs to the Static and Dynamic Component Encoders, which produce five nonnegative scores and signed expression and pose scores, respectively. Component Score Fusion yields the overall rating and per-image weighted contributions. Demographic Conditioning provides a shared embedding to the component-specific feature-wise linear modulation (FiLM)~\cite {perez2018film} layers}{figure.2}{}}
\newlabel{main:sec:static_encoder}{{\mbox  {III-D}}{4}{Static Component Encoder}{subsection.3.4}{}}
\newlabel{main:sec:dynamic_encoder}{{\mbox  {III-E}}{4}{Dynamic Component Encoder}{subsection.3.5}{}}
\newlabel{main:sec:score_fusion}{{\mbox  {III-F}}{4}{Component Score Fusion}{subsection.3.6}{}}
\newlabel{main:eq:score_assembly}{{8}{5}{Component Score Fusion}{equation.8}{}}
\newlabel{main:eq:frozen_fusion_fit}{{9}{5}{Component Score Fusion}{equation.9}{}}
\newlabel{main:sec:training_scheme}{{\mbox  {III-G}}{5}{Joint Learning and Frozen Fusion Fitting}{subsection.3.7}{}}
\newlabel{main:eq:training_objective}{{19}{5}{Static-score balance}{equation.19}{}}
\newlabel{main:sec:experiments}{{IV}{5}{Experiments}{section.4}{}}
\newlabel{main:fig:joint_training}{{3}{6}{Two-stage training in DisFace3DNet. Stage~1 jointly trains seven component routes using ground-truth (GT) ratings, scalar knowledge distillation (KD) from FPEM~\cite {li2025facial}, and GPT-5.5 weak labels~\cite {openai2026gpt55}. The provisional score $\tilde y_n$ and distribution head $\pi $ receive the indicated loss terms. Stage~2 freezes the network and fits fusion coefficients on the standardized static/dynamic outputs through $\mathcal {L}_{\mathrm {fit}}$}{figure.3}{}}
\newlabel{main:sec:evaluation_metrics}{{\mbox  {IV-B}}{6}{Evaluation Metrics}{subsection.4.2}{}}
\newlabel{main:sec:implementation}{{\mbox  {IV-C}}{6}{Implementation Details}{subsection.4.3}{}}
\newlabel{main:tab:main_performance}{{I}{7}{Overall attractiveness prediction on SCUT-FBP5500~\cite {Liang2018SCUT}, grouped by model category}{table.1}{}}
\newlabel{main:sec:component_results}{{\mbox  {V-B}}{7}{Component Score Prediction}{subsection.5.2}{}}
\newlabel{main:fig:prediction_distributions}{{4}{8}{DisFace3DNet and FPEM~\cite {li2025facial} prediction distributions for 1,000 held-out images. White dots and black bars indicate medians and interquartile ranges. Paired $t$-test $p$-values are unadjusted overall and Holm-adjusted across the four groups; ns denotes $p\geq 0.05$}{figure.4}{}}
\newlabel{main:fig:prediction_examples}{{5}{8}{Qualitative prediction examples. Four images per group are ordered by increasing human mean rating. Blue/red encodes lower/higher ratings on a fixed 1--5 scale}{figure.5}{}}
\newlabel{main:fig:identity_skin_3d}{{6}{8}{3D identity and skin examples: (a) Asian Male, (b) Asian Female, (c) Caucasian Male, (d) Caucasian Female. Each row shows three lower-score and three higher-score heads. Identity displays neutral geometry; skin uses personal-albedo-guided color and FFHQ-UV detail for display. Labels give raw component scores on $[0,1]$}{figure.6}{}}
\newlabel{main:eq:contribution_share}{{20}{8}{Component contribution variation}{equation.20}{}}
\newlabel{main:fig:component_output_examples}{{7}{9}{Component-score examples by benchmark group (columns), with three lower- and three higher-score images per component. Labels show $S_k$ for static components ($[0,1]$), $10S_k$ for expression, and $100S_k$ for pose. Displayed expression/pose ranges are $[-0.48,+0.80]$/$[-0.29,+0.65]$}{figure.7}{}}
\newlabel{main:fig:component_score_distributions}{{8}{9}{Component-score distributions for all 5,500 held-out SCUT-FBP5500 images and the four benchmark groups. Static scores lie in $[0,1]$; expression and pose use signed axes. Density curves have equal peak heights, and labels report mean $\pm $ sample SD. Scores precede fold-specific standardization and fusion}{figure.8}{}}
\newlabel{main:tab:component_contributions}{{II}{10}{Relative component contribution magnitudes (\%) with 95\% image-bootstrap intervals conditional on the frozen models. Each column sums to 100\% before rounding. Identity denotes facial shape and structure. AM, AF, CM, and CF denote Asian Male, Asian Female, Caucasian Male, and Caucasian Female, respectively}{table.2}{}}
\newlabel{main:fig:human_alignment}{{9}{10}{Component-specific human evaluation with 20 participants. (a) Restyled skin-trial interface with the original stimulus pair and response options; no response is shown. (b) Pairwise agreement. Yellow circles: fraction of decisive responses matching the model's score ordering. Blue diamonds: mean per-response agreement fraction with other participants on the same component and image pair. Both exclude unsure responses and repeats; diamonds require a decisive peer. Bars: 95\% participant-clustered bootstrap intervals. Vertical line: 50\% agreement between independent fair binary choices}{figure.9}{}}
\newlabel{main:sec:human_evaluations}{{\mbox  {V-C}}{10}{Human Evaluation}{subsection.5.3}{}}
\newlabel{main:sec:ablations}{{\mbox  {V-D}}{10}{Ablation Studies}{subsection.5.4}{}}
\newlabel{main:tab:training_signal_ablation}{{III}{11}{Five-fold ablations of component scoring, training objectives, and training strategy. Metric summaries are mean $\pm $ sample SD across folds. $\Delta $PCC is DisFace3DNet minus the variant (positive favors DisFace3DNet), with marginal 95\% paired image-bootstrap CIs}{table.3}{}}
\newlabel{main:fig:head_candidate_selection}{{10}{11}{Illustrative applications of DisFace3DNet. Component reference scores support (a) digital-human and bio-inspired robot face design, (b) beauty-filter assessment for livestreaming, photography, and social media, and (c) hairstyle design, salon consultation, and wig try-on}{figure.10}{}}
\newlabel{main:sec:applications}{{VI}{11}{Applications}{section.6}{}}
\newlabel{main:sec:conclusion}{{VII}{12}{Conclusion}{section.7}{}}

